Paloma: A Benchmark for Evaluating Language Model Fit

Evaluations of language models (LMs) commonly report perplexity on monolithic data held out from training. Implicitly or explicitly, this data is composed of domains--varying distributions of language. We introduce Perplexity Analysis for Language Model Assessment (Paloma), a benchmark to measure LM fit to 546 English and code domains, instead of assuming perplexity on one distribution extrapolates to others. We include two new datasets of the top 100 subreddits (e.g., r/depression on Reddit) and programming languages (e.g., Java on GitHub), both sources common in contemporary LMs. With our benchmark, we release 6 baseline 1B LMs carefully controlled to provide fair comparisons about which pretraining corpus is best and code for others to apply those controls to their own experiments. Our case studies demonstrate how the fine-grained results from Paloma surface findings such as that models pretrained without data beyond Common Crawl exhibit anomalous gaps in LM fit to many domains or that loss is dominated by the most frequently occurring strings in the vocabulary.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}
\usepackage{dsfont}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
% \def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/source_statistics_old.tex <==
\begin{tabular}{llrrrrr}
\toprule
Purpose & Source & Validation & Test & Combined & Domains & Tokens per Split per Domain \\
\midrule
\multirow[c]{8}{1.25cm}{Standard language modeling benchmarks} & \cFour & 1,000,000 & 1,000,000 & 2,000,000 & 1 & 1,000,000 \\
&\mCFourEn & 1,000,000 & 1,000,000 & 2,000,000 & 1 & 1,000,000 \\
&\pile & 2,199,944 & 2,199,333 & 4,399,277 & 22 & 99,984 \\
&\wikitext & 247,969 & 283,134 & 531,103 & 1 & 265,552 \\
&\ptb & \textbf{89,917} & \textbf{101,818} & \textbf{191,735} & 1 & \textbf{95,868} \\
&\redPajama & 699,946 & 700,000 & 1,399,946 & 7 & 99,996 \\
&\falcon & 1,000,000 & 1,000,000 & 2,000,000 & 1 & 1,000,000 \\
&\dolma & 2,999,998 & 2,994,903 & 5,994,901 & 6 & 499,575 \\ \cmidrule{2-7}

\multirow[c]{5}{1.25cm}{Fine-grained domain benchmarks} & \mTwoDTwoSTwoORC & 16,691,625 & 16,682,726 & 33,374,351 & 167 & 99,923 \\
&\mTwoDTwoWiki & 4,890,146 & 4,890,573 & 9,780,719 & 49 & 99,803 \\
&\cFourOneHundredDomains & 9,795,511 & 9,813,881 & 19,609,392 & 99 & 99,037 \\
&\dolmaOneHundredSubreddits & 9,679,376 & 9,680,887 & 19,360,263 & 100 & 96,801 \\
&\stackOneHundredLanguages & 9,999,707 & 9,999,906 & 19,999,613 & 100 & 99,998 \\  \cmidrule{2-7}

\multirow[c]{3}{1.25cm}{Disparities between communities} & \ice & 7,290,880 & 7,236,065 & 14,526,945 & 17 & 427,263 \\
& \twitterAAE & 722,905 & 718,358 & 1,441,263 & 2 & 360,316 \\
& \manosphere & 1,000,000 & 999,915 & 1,999,915 & 9 & 111,106 \\  \cmidrule{2-7}

\multirow[c]{2}{1.25cm}{Fringe sources} & \gab & 1,000,000 & 1,000,000 & 2,000,000 & 1 & 1,000,000 \\
& \fourChan & 1,000,000 & 1,000,000 & 2,000,000 & 1 & 1,000,000 \\ \cmidrule{2-7}
& \pplSuite{} & 71,307,924 & 71,301,499 & 142,609,423 & 585 & 121,888 \\
\bottomrule
\end{tabular}


==> tables/subsetting_variability.tex <==
% \begin{table*}[]
% \tiny
% \centering
\begin{tabular}{llllllll}
\toprule
 &      & \multicolumn{6}{c}{Evaluation Subsample Tokens}                                            \\
 &      & 100k         & 250k         & 500k         & 1000k        & 4000k        & 8000k        \\
\cmidrule{3-8}
\multirow{4}{*}{\rotatebox[origin=c]{90}{Train Toks}} & 4B & 41.11 ± 2.31 & 41.92 ± 1.63 & 42.10 ± 1.25 & 41.99 ± 0.80 & 42.06 ± 0.39 & 42.06 ± 0.24 \\
 & 25B  & 21.31 ± 1.18 & 21.69 ± 0.82 & 21.80 ± 0.64 & 21.77 ± 0.42 & 21.79 ± 0.20 & 21.80 ± 0.13 \\
 & 86B  & 17.96 ± 0.99 & 18.27 ± 0.67 & 18.37 ± 0.53 & 18.36 ± 0.35 & 18.37 ± 0.17 & 18.37 ± 0.11 \\
 & 300B & 15.72 ± 0.87 & 15.95 ± 0.56 & 16.03 ± 0.44 & 16.03 ± 0.31 & 16.02 ± 0.14 & 16.02 ± 0.09 \\
\bottomrule
\end{tabular}
% \caption{Average perplexity over 20 subsets of \cFour{} validation data using Pythia 1.4B checkpoints. Token counts are for the GPT-NeoX-20B tokenizer \cite{gpt-neo} used by Pythia.}
% \label{tab:subsetting_variability}
% \end{table*}

==> tables/tmp/domains_100_PLs.tex <==
\begin{tabular}{p{6.5cm}}
\toprule

00\_text, 01\_markdown, 02\_c, 03\_php, 04\_java, 05\_c++, 06\_python, 07\_javascript, 08\_html, 09\_c\#, 10\_yaml, 11\_go, 12\_typescript, 13\_xml, 14\_css, 15\_jupyter-notebook, 16\_rust, 17\_unity3d-asset, 18\_gettext-catalog, 19\_ruby, 20\_vue, 21\_sql, 22\_swift, 23\_kotlin, 24\_scala, 25\_scss, 26\_tex, 27\_dart, 28\_kicad, 29\_shell, 30\_smali, 31\_lua, 32\_restructuredtext, 33\_perl, 34\_diff, 35\_ini, 36\_jsx, 37\_haskell, 38\_gnuplot, 39\_postscript, 40\_groff, 41\_turtle, 42\_fortran, 43\_makefile, 44\_mathematica, 45\_pascal, 46\_common-lisp, 47\_gas, 48\_vhdl, 49\_julia, 50\_edn, 51\_visual-basic, 52\_powershell, 53\_g-code, 54\_ocaml, 55\_java-server-pages, 56\_solidity, 57\_graphviz-dot, 58\_less, 59\_twig, 60\_asciidoc, 61\_groovy, 62\_llvm, 63\_hcl, 64\_html+erb, 65\_erlang, 66\_elixir, 67\_eagle, 68\_arduino, 69\_coffeescript, 70\_toml, 71\_cuda, 72\_nix, 73\_smalltalk, 74\_cmake, 75\_actionscript, 76\_glsl, 77\_systemverilog, 78\_haxe, 79\_f\#, 80\_max, 81\_objective-c++, 82\_standard-ml, 83\_dockerfile, 84\_emacs-lisp, 85\_scheme, 86\_clojure, 87\_handlebars, 88\_smarty, 89\_logos, 90\_stata, 91\_yacc, 92\_nimrod, 93\_tcl, 94\_viml, 95\_asp, 96\_protocol-buffer, 97\_r, 98\_cython, 99\_mediawiki \\
\bottomrule
\end{tabular}


==> tables/tmp/domains_100_Subreddits.tex <==
\begin{tabular}{p{6.5cm}}
\toprule

00\_AskReddit, 01\_politics, 02\_AmItheAsshole, 03\_worldnews, 04\_relationships, 05\_relationship\_advice, 06\_news, 07\_leagueoflegends, 08\_todayilearned, 09\_TwoXChromosomes, 10\_personalfinance, 11\_changemyview, 12\_unpopularopinion, 13\_movies, 14\_Games, 15\_nba, 16\_pics, 17\_gaming, 18\_soccer, 19\_nfl, 20\_explainlikeimfive, 21\_conspiracy, 22\_atheism, 23\_AskMen, 24\_videos, 25\_sex, 26\_raisedbynarcissists, 27\_NoStupidQuestions, 28\_DestinyTheGame, 29\_anime, 30\_DnD, 31\_ukpolitics, 32\_funny, 33\_europe, 34\_canada, 35\_Christianity, 36\_SquaredCircle, 37\_AskWomen, 38\_legaladvice, 39\_JUSTNOMIL, 40\_technology, 41\_IAmA, 42\_wow, 43\_Parenting, 44\_exmormon, 45\_AdviceAnimals, 46\_childfree, 47\_unitedkingdom, 48\_ffxiv, 49\_dndnext, 50\_ADHD, 51\_loseit, 52\_asoiaf, 53\_BabyBumps, 54\_Advice, 55\_australia, 56\_CFB, 57\_offmychest, 58\_PublicFreakout, 59\_TrueOffMyChest, 60\_science, 61\_magicTCG, 62\_asktransgender, 63\_DotA2, 64\_neoliberal, 65\_whowouldwin, 66\_depression, 67\_WTF, 68\_pathofexile, 69\_PoliticalDiscussion, 70\_Libertarian, 71\_PurplePillDebate, 72\_Fitness, 73\_books, 74\_dogs, 75\_pcmasterrace, 76\_teenagers, 77\_stopdrinking, 78\_Overwatch, 79\_television, 80\_buildapc, 81\_askscience, 82\_programming, 83\_Guildwars2, 84\_cars, 85\_formula1, 86\_sysadmin, 87\_hockey, 88\_india, 89\_SubredditDrama, 90\_DMAcademy, 91\_dating\_advice, 92\_Catholicism, 93\_Drugs, 94\_trees, 95\_boardgames, 96\_Conservative, 97\_Futurology, 98\_beyondthebump, 99\_weddingplanning \\
\bottomrule
\end{tabular}


==> tables/tmp/domains_C4_100_Domains.tex <==
\begin{tabular}{p{6.5cm}}
\toprule

100\_www.ign.com, 10\_www.eventbrite.com, 11\_link.springer.com, 12\_www.chicagotribune.com, 13\_www.foxnews.com, 14\_www.aljazeera.com, 15\_www.dailymail.co.uk, 16\_www.ncbi.nlm.nih.gov, 17\_www.express.co.uk, 18\_en.m.wikipedia.org, 19\_www.cnet.com, 1\_www.nytimes.com, 20\_www.telegraph.co.uk, 21\_www.theatlantic.com, 22\_forums.macrumors.com, 23\_www.oreilly.com, 24\_www.washingtonpost.com, 25\_www.zdnet.com, 26\_www.foxbusiness.com, 27\_www.reuters.com, 28\_www.ibtimes.co.uk, 29\_www.rt.com, 2\_en.wikipedia.org, 30\_www.prweb.com, 31\_www.deviantart.com, 32\_www.si.com, 33\_www.bbc.com, 34\_github.com, 35\_nypost.com, 36\_itunes.apple.com, 37\_www.instructables.com, 38\_www.youtube.com, 39\_www.booking.com, 40\_www.etsy.com, 41\_www.marketwired.com, 42\_sites.google.com, 43\_www.baltimoresun.com, 44\_www.agreatertown.com, 45\_www.npr.org, 46\_www.fool.com, 47\_www.tripadvisor.com, 48\_www.bbc.co.uk, 49\_lists.w3.org, 4\_www.latimes.com, 50\_mashable.com, 51\_disneyparksmomspanel.disney.go.com, 52\_www.cnbc.com, 53\_answers.sap.com, 54\_homestars.com, 55\_www.hindustantimes.com, 56\_www.reference.com, 57\_www.city-data.com, 58\_medium.com, 59\_app-wiringdiagram.herokuapp.com, 5\_www.theguardian.com, 60\_www.csmonitor.com, 61\_www.adweek.com, 62\_docs.microsoft.com, 63\_www.yahoo.com, 64\_www.thesun.co.uk, 65\_www.nydailynews.com, 66\_www.dailystar.co.uk, 67\_fineartamerica.com, 68\_www.kickstarter.com, 69\_uk.reuters.com, 6\_www.huffpost.com, 70\_www.insiderpages.com, 71\_www.inquisitr.com, 72\_lists.debian.org, 73\_www.straitstimes.com, 74\_www.cbsnews.com, 75\_simple.wikipedia.org, 76\_deadline.com, 77\_www.androidheadlines.com, 78\_www.wired.com, 79\_www.bustle.com, 7\_patents.google.com, 80\_premium.wpmudev.org, 81\_www.librarything.com, 82\_mail-archives.apache.org, 83\_scholars.duke.edu, 84\_www.glassdoor.com, 85\_www.pcworld.com, 86\_www.shutterstock.com, 87\_myemail.constantcontact.com, 88\_www.eventbrite.co.uk, 89\_www.fastcompany.com, 8\_www.businessinsider.com, 90\_www.firstpost.com, 91\_www.entrepreneur.com, 92\_www.breitbart.com, 93\_techcrunch.com, 94\_www.nme.com, 95\_www.ndtv.com, 96\_finance.yahoo.com, 97\_archives.lib.state.ma.us, 98\_www.gsmarena.com, 99\_www.lonelyplanet.com, 9\_www.forbes.com \\
\bottomrule
\end{tabular}


==> tables/tmp/domains_Dolma_V1.5.tex <==
\begin{tabular}{c}
\toprule

books, common-crawl, pes2o, reddit\_uniform, stack\_uniform, wiki \\
\bottomrule
\end{tabular}


==> tables/tmp/domains_ICE.tex <==
\begin{tabular}{p{6.5cm}}
\toprule

CANADA\_S\_ALL, CANADA\_W\_ALL, EAST\_AFRICA\_S\_ALL, EAST\_AFRICA\_W\_ALL, HONG\_KONG\_S\_ALL, HONG\_KONG\_W\_ALL, INDIA\_S\_ALL, INDIA\_W\_ALL, IRELAND\_S\_ALL, IRELAND\_W\_ALL, JAMAICA\_S\_ALL, JAMAICA\_W\_ALL, PHILIPPINES\_S\_ALL, PHILIPPINES\_W\_ALL, SINGAPORE\_S\_ALL, SINGAPORE\_W\_ALL, USA\_W\_ALL \\
\bottomrule
\end{tabular}


==> tables/tmp/domains_M2D2_S2ORC.tex <==
\begin{tabular}{p{6.5cm}}
\toprule

Art, Philosophy, astro-ph, astro-ph.CO, astro-ph.EP, astro-ph.GA, astro-ph.HE, astro-ph.IM, astro-ph.SR, astro-ph\_l1, atom-ph, chem-ph, cond-mat, cond-mat.dis-nn, cond-mat.mes-hall, cond-mat.mtrl-sci, cond-mat.other, cond-mat.quant-gas, cond-mat.soft, cond-mat.stat-mech, cond-mat.str-el, cond-mat.supr-con, cond-mat\_l1, cs.AI, cs.AR, cs.CC, cs.CE, cs.CG, cs.CL, cs.CR, cs.CV, cs.CY, cs.DB, cs.DC, cs.DL, cs.DM, cs.DS, cs.ET, cs.FL, cs.GL, cs.GR, cs.GT, cs.HC, cs.IR, cs.LG, cs.LO, cs.MA, cs.MM, cs.MS, cs.NA, cs.NE, cs.NI, cs.OH, cs.OS, cs.PF, cs.PL, cs.RO, cs.SC, cs.SD, cs.SE, cs.SI, cs.SY, cs\_l1, econ.EM, econ.TH, econ\_l1, eess.AS, eess.IV, eess.SP, eess\_l1, gr-qc, hep-ex, hep-lat, hep-ph, hep-th, math.AC, math.AG, math.AP, math.AT, math.CA, math.CO, math.CT, math.CV, math.DG, math.DS, math.FA, math.GM, math.GN, math.GR, math.GT, math.HO, math.KT, math.LO, math.MG, math.NA, math.NT, math.OA, math.OC, math.PR, math.QA, math.RA, math.RT, math.SG, math.SP, math\_l1, nlin.AO, nlin.CD, nlin.CG, nlin.PS, nlin.SI, nlin\_l1, nucl-ex, nucl-th, physics.acc-ph, physics.ao-ph, physics.app-ph, physics.atm-clus, physics.atom-ph, physics.bio-ph, physics.chem-ph, physics.class-ph, physics.comp-ph, physics.data-an, physics.ed-ph, physics.flu-dyn, physics.gen-ph, physics.geo-ph, physics.hist-ph, physics.ins-det, physics.med-ph, physics.optics, physics.plasm-ph, physics.pop-ph, physics.soc-ph, physics.space-ph, physics\_l1, plasm-ph, q-bio, q-bio.BM, q-bio.CB, q-bio.GN, q-bio.MN, q-bio.NC, q-bio.OT, q-bio.PE, q-bio.QM, q-bio.SC, q-bio.TO, q-bio\_l1, q-fin.CP, q-fin.EC, q-fin.GN, q-fin.MF, q-fin.PM, q-fin.PR, q-fin.RM, q-fin.ST, q-fin.TR, q-fin\_l1, quant-ph, stat.AP, stat.CO, stat.ME, stat.ML, stat.OT, stat\_l1, supr-con \\
\bottomrule
\end{tabular}


==> tables/tmp/domains_M2D2_Wikipedia.tex <==
\begin{tabular}{p{6.5cm}}
\toprule

Culture\_and\_the\_arts, Culture\_and\_the\_arts\_\_Culture\_and\_Humanities, Culture\_and\_the\_arts\_\_Games\_and\_Toys, Culture\_and\_the\_arts\_\_Mass\_media, Culture\_and\_the\_arts\_\_Performing\_arts, Culture\_and\_the\_arts\_\_Sports\_and\_Recreation, Culture\_and\_the\_arts\_\_The\_arts\_and\_Entertainment, Culture\_and\_the\_arts\_\_Visual\_arts, General\_referece, General\_referece\_\_Further\_research\_tools\_and\_topics, General\_referece\_\_Reference\_works, Health\_and\_fitness, Health\_and\_fitness\_\_Exercise, Health\_and\_fitness\_\_Health\_science, Health\_and\_fitness\_\_Human\_medicine, Health\_and\_fitness\_\_Nutrition, Health\_and\_fitness\_\_Public\_health, Health\_and\_fitness\_\_Self\_care, History\_and\_events, History\_and\_events\_\_By\_continent, History\_and\_events\_\_By\_period, History\_and\_events\_\_By\_region, Human\_activites, Human\_activites\_\_Human\_activities, Human\_activites\_\_Impact\_of\_human\_activity, Mathematics\_and\_logic, Mathematics\_and\_logic\_\_Fields\_of\_mathematics, Mathematics\_and\_logic\_\_Logic, Mathematics\_and\_logic\_\_Mathematics, Natural\_and\_physical\_sciences, Natural\_and\_physical\_sciences\_\_Biology, Natural\_and\_physical\_sciences\_\_Earth\_sciences, Natural\_and\_physical\_sciences\_\_Nature, Natural\_and\_physical\_sciences\_\_Physical\_sciences, Philosophy\_and\_thinking, Philosophy\_and\_thinking\_\_Philosophy, Philosophy\_and\_thinking\_\_Thinking, Religion\_and\_belief\_systems, Religion\_and\_belief\_systems\_\_Allah, Religion\_and\_belief\_systems\_\_Belief\_systems, Religion\_and\_belief\_systems\_\_Major\_beliefs\_of\_the\_world, Society\_and\_social\_sciences, Society\_and\_social\_sciences\_\_Social\_sciences, Society\_and\_social\_sciences\_\_Society, Technology\_and\_applied\_sciences, Technology\_and\_applied\_sciences\_\_Agriculture, Technology\_and\_applied\_sciences\_\_Computing, Technology\_and\_applied\_sciences\_\_Engineering, Technology\_and\_applied\_sciences\_\_Transport \\
\bottomrule
\end{tabular}


==> tables/tmp/domains_Manosphere.tex <==
\begin{tabular}{c}
\toprule

avfm, incels, love\_shy, mgtow, pua\_forum, red\_pill\_talk, reddit, rooshv, the\_attraction \\
\bottomrule
\end{tabular}


==> tables/tmp/domains_RedPajama.tex <==
\begin{tabular}{c}
\toprule

arxiv, books, c4, commoncrawl, github, stackexchange, wikipedia \\
\bottomrule
\end{tabular}


==> tables/tmp/domains_The_Pile.tex <==
\begin{tabular}{p{6.5cm}}
\toprule

ArXiv, BookCorpus2, Books3, DM\_Mathematics, Enron\_Emails, EuroParl, FreeLaw, Github, Gutenberg\_PG-19, HackerNews, NIH\_ExPorter, OpenSubtitles, OpenWebText2, PhilPapers, Pile-CC, PubMed\_Abstracts, PubMed\_Central, StackExchange, USPTO\_Backgrounds, Ubuntu\_IRC, Wikipedia\_en, YoutubeSubtitles \\
\bottomrule
\end{tabular}


==> tables/tmp/domains_Twitter_AAE.tex <==
\begin{tabular}{c}
\toprule

AA, white \\
\bottomrule
\end{tabular}

